PrettyCat: Adaptive guarantee-controlled software partitioning of security protocols

One single error can result in a total compromise of all security in today's large, monolithic software. Partitioning of software can help simplify code-review and verification, whereas isolated execution of software-components limits the impact of incorrect implementations. However, existing application partitioning techniques are too expensive, too imprecise, or involve unsafe manual steps. An automatic, yet safe, approach to dissect security protocols into component-based systems is not available. We present a method and toolset to automatically segregate security related software into an indefinite number of partitions, based on the security guarantees required by the deployed cryptographic building blocks. As partitioning imposes communication overhead, we offer a range of sound performance optimizations. Furthermore, by applying our approach to the secure messaging protocol OTR, we demonstrate its applicability and achieve a significant reduction of the trusted computing base. Compared to a monolithic implementation, only 29% of the partitioned protocol requires confidentiality guarantees with a process overhead comparable to common sandboxing techniques.

==> parts/theory.tex <==
\section{\label{sec:framework}Modeling framework}

\subsection{Primitives}

A primitive $\PR{}$ is defined by its name $np$, its input ports $\T_{in}$,
its output ports $\T_{out}$ and its rule $\R$.

\begin{align}
    \PR_{np} &= (\T_{in}, \T_{out}, \R)
\end{align}

The set $\T_{in}$ contains the variable names of the input ports a primitive
can receive messages on. $\T_{out}$ holds the output port variables a
primitive can use for sending out messages, respectively.

Port variables are local to the primitive and the direction, i.e. different
primitives can have identical port variable and input ports may use the same
variable names as output ports. Ports are free variables that are later bound
specific channel variables.

The rule $\R$ states the relationship between the guarantees of input and
output ports. Output variables are marked with a arrow symbol, such that a
variable with the name ``Result'' is written as $\outvar{Result}$. Input
variables have no special marking, such that ``Data" input port is referred as
$\invar{Data}$. 

The set $\NameP$ denotes unique primitive names and $\PS$ the set of existing
primitives:

\begin{align}
    \PS    &= \{\PR_{np} | np \in \NameP\} \\
    \NameP &= \{np | \text{name of a primitive}\}
\end{align}

\subsection{Instances}

A network implementing a cryptographic protocol typically requires multiple
instances of the same primitive. A primitive $\PR_{np}$ is instantiated by
binding its free variables in $\T_{in}$ and $\T_{out}$ to unique global names.
Additionally, the rule $\R$ is also instantiated as described in section
\nameref{subsec:rules}.

Applying the described transformation results in an instance with a global,
unique name $ni$:

\begin{align}
    \I_{ni} &= (np, \T^{\prime}_{in}, \T^{\prime}_{out}, \R^{\prime}) | np \in \NameP, ni \in \NameI \\
      \NameI &= \{n | \text{name of an instance}\}
\end{align}

Let $\name: \NameI \times (\T_{in} \cup \T_{out})$ be a bijective function that
takes a unique instance name $ni$ and a free, local variable $v$ and outputs a
globally unique variable name $\name(ni, v)$. Applying this function to
$\T_{in}$ and $\T_{out}$ results in $\T^{\prime}_{in}$ and $\T^{\prime}_{out}$
containing only bound, global variables.

\begin{align}
    \T^{\prime}_{in}  &= \{ \name(ni, j) | j\in\T_{in} \} \\
    \T^{\prime}_{out} &= \{ \name(ni, k) | k\in\T_{out} \}
\end{align}

\subsection{\label{subsec:rules}Rules}

A rule is a boolean expression of a primitive defining the relation between
integrity and confidentiality guarantees of its input and output ports using
free variables. We can refer to the integrity guarantee of an input variable
$\invar{Data}$ as $\intg{\invar{Data}}$ and state the confidentiality guarantee
as $\conf{\invar{Data}}$. The guarantees for output variables are defined
accordingly.

Using $\name$, we bind the free port variables in the rule $\R$ for a specific
instance name $ni$.  The bound rule $\R^{\prime}$ is created by replacing every
occurrence of an output variable $o$ in $\R$ by $\name(ni, o)$ and every
occurrence of an input variable $i$ by $\name(ni, i)$:

\begin{align}
    \R^{\prime} = \R[&i := \name (ni, i) | \forall i \in \T_{in}, \nonumber\\
                     &o := \name (ni, o) | \forall o \in \T_{out}]
\end{align}

\subsection{\label{subsec:channels}Channels}

A channel $\C_{src, p_{out}, dst, p_{in}}$ connects an output port of a source
instance $\I_{src}$ with an input port of a destination instance $\I_{dst}$.
The specified ports $p_{out} \in \T_{out}$ and $p_{in} \in \T_{in}$ are defined
in the respective primitives $\I_{src}$ and $\I_{dsc}$ were instantiated from.
Specifically, the instances might be derived from different primitives.

\begin{align}
    \C_{src,p_{out},dst,p_{in}} = (src, p_{out}, dst, p_{in}, \R^{\prime}_c), \nonumber\\
    src, dst \in \NameI, src \neq dst, p_{out} \text{ in } \I_{src}, p_{in} \text{ in } \I_{dst}
\end{align}

All channels have the same channel rule $\R_c$ with only two free variables,
$\outv$ and $\inv$. It represents the output port of a sending instance and the
input port of a receiving instances, respectively. It states that the
confidentiality guarantee of the connected ports must be equivalent. The same
equivalence holds for integrity.

\begin{align}
    \R_c = \intg{\outvar{\outv}} \Leftrightarrow \intg{\invar{\inv}}
            \land{} \conf{\outvar{\outv}} \Leftrightarrow \conf{\invar{\inv}}
\end{align}

$\R^{\prime}_c$ is the bound version of the generic channel rule $\R_c$ for a
specific channel $\C_{src,p_{out},dst,p_{in}}$. The free variable $\outv$ in
$\R_c$ is bound to the unique global name $\name(src, p_{out})$ of the output
port $p_{out}$. $\inv$ is bound to the unique global name $\name(dst, p_{in})$,
respectively:

\begin{align}
    \R^{\prime}_c = \R_c[In &:= \name(src, p_{out}),\nonumber\\Out &:= \name(dst, p_{in})]
\end{align}

% _{c,src,p_o,dst,p_i}

\subsection{\label{subsec:guarantees}Guarantees}

While different ports of a primitive may require different guarantees, there is
an overall guarantee an instance requires from the execution environment. This
guarantee is determined by the respective port guarantees as follows.

The confidentiality guarantee $\conf{\I}$ of some instance $\I$ is determined
by the disjunction of the confidentiality guarantees of its input and output
ports:

\begin{align}
    \conf{\I} = \bigvee_{\mathclap{p\in\T^\prime_{in}\cup\T^\prime_{out}}}\conf{p}\qquad\T^\prime_{in}, \T^\prime_{out}\mathrel{in} \I
    \label{eq:inst_conf}
\end{align}

The integrity guarantee $\intg{\I}$ for an instance $\I$ is defined accordingly:

\begin{align}
    \intg{\I} = \bigvee_{\mathclap{p\in\T^\prime_{in}\cup\T^\prime_{out}}}\intg{p}\qquad\T^\prime_{in}, \T^\prime_{out}\mathrel{in} \I
    \label{eq:inst_intg}
\end{align}

\subsection{Network}

The network with the name $n$ is fully defined by its instances the
channels between them and the domains the instances belong to:

\begin{align}
    \NE_{n} &= (\II, \CS, \Dom) \\
    \II     &= \{\I_{ni}|ni \in \NameI\}
\end{align}

\begin{align}
    \CS = \{\C_{src,p_{out},dst,p_{in}} | src, dst &\in \NameI,\\
                                               src &\neq dst,\\
                               \name(src, p_{out}) &\text{ in } \I_{src},\\
                                \name(dst, p_{in}) &\text{ in } \I_{dst} \}
\end{align}

\subsection{\label{subsec:partitioning}Partitioning}

Partitioning is the process of grouping connected instances in a network into
protection domains. Instances A protection domain $\PD$ is a set of instances
in $\II$ executing without isolation from each other:

\begin{align}
    \PD_i = \{\I_j | \I \in \II\}
\end{align}

An instance belongs to exactly one protection domain $\PD$ in the set $\Dom$ of
all protection domains in a network:

\begin{align}
    \Dom = \{\PD_1 \dots \PD_n | \forall I_j, k, l:  I_j \in \PD_k, \I_j \notin \PD_l, k \ne l\}
\end{align}

As we need to iterate the network along its channels to find partitions, we
define functions that return the instances connected to the ports of an
instance. The instance connected to an input port of an instance is called its
predecessor, the instance connected to an output port is called its successor.

\begin{align}
    \gpred(\NE, \I, p) = 
    \begin{cases}
        s    & \text{if } C_{s,po,d,pi} \in \CS \mathrel{in} \NE: I=d, p=pi \\
        \bot & \text{otherwise}
    \end{cases}
\end{align}

\begin{align}
    \gsucc(\NE, \I, p) = 
    \begin{cases}
        d    & \text{if } C_{s,po,d,pi} \in \CS \mathrel{in} \NE: I=s, p=po \\
        \bot & \text{otherwise}
    \end{cases}
\end{align}

The partition an instance is assigned to is determined as follows:

\begin{align}
    \gpart(\Dom, \I) = 
    \begin{cases}
        p    & \text{if } \exists p: \I\in\PD_p\mathrel{in}\Dom \\
        \bot & \text{otherwise}
    \end{cases}
\end{align}

The guarantees required for a partition $\PD_{p}$ are determined like the
guarantees for instances (cf. \Cref{eq:inst_conf}, \Cref{eq:inst_intg}):

\begin{align}
    \conf{\PD_p} & = \bigvee\conf{\I_i}\qquad \I_i\in\PD_p \\
    \intg{\PD_p} & = \bigvee\intg{\I_i}\qquad \I_i\in\PD_p
\end{align}

The simplest approach to partitioning is to put connected instances with
identical guarantees into the same partition using algorithm
\Cref{algo:basic}. The basic idea is to iterate over all instances in the
network. For each instance, check whether it is assigned to a partition
already. Otherwise, assign it to a new partition and iterate over all its
predecessors and successors and try to assign it to the same partition. 

The above algorithm assigns instances to the same partition only if they
require exactly the same guarantees. Consequently, each instance of a
\emph{Const} primitive connected to a cryptographic primitive will end up in
its own partition. The reason is, that \emph{Const} primitives never require
confidentiality, while cryptographic primitives typically do. 

Providing more guarantees to primitives than required, obviously poses no
security problem. It can, however, increase the TCB. We argue, that upgrading
single \emph{Const} primitives to the extended guarantees of the partition they
are connected results only in a minor increase of the TCB. Those primitives
will typically have a very simple implementation, like accessing a piece of
read-only memory.

The following algorithm merges \emph{Const} primitives in a network with the
partition they are connected to, given it requires less guarantees. For the
algorithm, it is useful to define a function to check the name of the primitive
the instance was derived from:

\begin{align}
    \gtype(\I, t) = t \equiv np \mathrel{in} \I
\end{align}

As we will change the domain an instance is assigned to, we need an update
function that inserts the instance to its target domain in $\Dom$ and removes
it from its old domain:

\begin{align}
    \gupdate(\Dom, \I, d) = \Dom & \setminus\left\{\PD_{\gpart(\Dom,\I)}, \PD_d\right\} \nonumber \\
                                 & \cup\left\{\PD_{\gpart(\Dom,\I)}\setminus\I, \PD_d\cup\I\right\}
\end{align}

With the above optimization, single constants are moved into compatible
domains. Another common pattern found in real-world protocols is a constant
which is branched into multiple instances of the same partition using a
\emph{Transform} primitive. As a branch typically only is a copy operation,
moving it into the target partition only slightly increases its TCB.

The extended algorithm is similar to algorithm \Cref{algo:const}. It
iterates over all instances of the network and for all \emph{Const} primitives
checks whether they are connected to a \emph{Transform} primitive. In that
case, for the \emph{Transform} it checks whether (a) all output ports are
connected to the same partition and (b) only one input port exists. For (a) we
define the function $\samepart$:

\begin{align}
    \samepart (\NE, \Dom, \I) =
    \begin{cases}
            q & \text{if } \exists q\forall r: \PD_q\equiv\PD_r, \\
              &            \qquad q,r\in\T_{out}\mathrel{in}I, \\
              &            \qquad\PD_q = \gpart(\Dom, \gsucc(\NE, \I, q)), \\
              &            \qquad\PD_r = \gpart(\Dom, \gsucc(\NE, \I, r)), \\
        \bot  & \text{otherwise}
    \end{cases}
\end{align}

If the guarantees for the \emph{Const} and for the \emph{Transform} primitives
are compatible with the target domain, both instances are moved to that domain.

% Eat this, Amr!

\subsection{Configuration}

\begin{figure}[h]
        \centering
        \tiny\sf
        \includegraphics[width=\linewidth]{images/error_xform_confidentiality_violation.pdf}
        \caption{Instances marked with dashed lines are involved in a contradiction
        found by solver (\emph{Integrity}: red, \emph{Integrity} and \emph{Confidentiality}: purple)}
        \label{fig:contradiction}
\end{figure}

\begin{figure}
        \begin{lstlisting}[style=XML]{Name=DHsec}
        <dhsec id="Calculate sec">
            <description>
                Calculate initiator secret value
            </description>
            <flow sarg="ssec" sink="Keystore" darg="data">
                <assert confidentiality="true">
                    The shared secret must be confidential.
                </assert>
            </flow>
        </dhsec>
        <env id="Keystore" confidentiality="true" code="print">
            <description>
                Output data to key store
            </description>
            <config mode="server" port="12001"/>
            <arg name="data"/>
        </env>
        \end{lstlisting}
        \caption{Excerpt from the model used in \Cref{subsubsec:simple_dh}}
        \label{fig:model_example}
\end{figure}

\subsection*{\label{subsec:example}Full example}

Using the notation introduced above, our minimal example from
\Cref{subsubsec:simple_enc} is defined as follows.

\subsubsection*{Primitives}

\begin{align*}
    \PR_{keystore} &= (\{\}, \{Key\},     \conf{\outvar{Key}} \equiv True \land \intg{\outvar{Key}} \equiv True) \\
    \PR_{user}     &= (\{\}, \{Msg\}, \conf{\outvar{Msg}} \equiv True) \\
    \PR_{internet} &= (\{Msg\}, \{\}, \conf{\invar{Msg}} \equiv False \land \intg{\invar{Msg}} \equiv False ) \\
    \PR_{const}    &= (\{\}, \{Const\},   True) \\
    \PR_{enc_ctr}  &= (\{Key, Ctr, Plain\}, \{Cipher\}, \R_{enc}) \\
    \R_{enc}       &= %\encryptrulenolabel
\end{align*}

\subsubsection*{Instances}

\begin{align*}
\I_{keystore,ks}  &= (\{\}, \{\name(ks, Key)\}, \R^{\prime}_{ks}) \\
\I_{user,us}      &= (\{\}, \{\name(us, Text)\}, \R^{\prime}_{us}) \\
\I_{internet,in}  &= (\{\name(in, Msg)\}, \{\}, \R^{\prime}_{in}) \\
\I_{const,iv}     &= (\{\}, \{\name(iv, Const)\}, \R^{\prime}_{iv}) \\
\I_{enc_ctr,enc}  &= (\{\name(enc, Key), \name(enc, Ctr),\\&\name(enc, Plain)\}, \\&\{\name(enc, Cipher)\}, \R^{\prime}_{enc}) \\
\end{align*}

\subsubsection*{Rules}

\begin{align}
\R^{\prime}_{ks}  &= \conf{\outvar{\name(ks, Key)}} \equiv True  \label{eq:ks1} \\
                  &\land \intg{\outvar{\name(ks, Key)}} \equiv True\label{eq:ks2} \\
\R^{\prime}_{us}  &= \conf{\outvar{\name(us, Text)}} \label{eq:us}\\
\R^{\prime}_{in}  &= \conf{\invar{\name(in, Msg)}} \equiv False \\
                  &\land \intg{\invar{\name(in, Msg)}} \equiv False \label{eq:in}\\
\R^{\prime}_{iv}  &= True \label{eq:iv} \\
\R^{\prime}_{enc} &= \intg{\outvar{\name(enc, Cipher)}} \rightarrow \intg{\invar{\name(enc, Plain)}} \label{eq:enc1}\\
                  &\land \intg{\invar{\name(enc, Key)}} \label{eq:enc2}\\
                  &\land \conf{\invar{\name(enc, Key)}} \label{eq:enc3}\\
                  &\land \intg{\invar{\name(enc, Ctr)}} \label{eq:enc4}
\end{align}

\subsubsection*{Channels}

\begin{align*}
    \CS = & \{(iv,Const,enc,Ctr,R^{\prime}_{c,iv,enc}), \\
          & (ks,Key,enc,Key,R^{\prime}_{c,ks,enc}), \\
          & (us,Text,enc,Plain,R^{\prime}_{c,us,enc}), \\
          & (enc,Cipher,in,Msg,R^{\prime}_{c,enc,in})\}
\end{align*}

\begin{align}
    \rc{iv}{Const}{enc}{Ctr} \\
    \rc{ks}{Key}{enc}{Key} \\
    \rc{us}{Msg}{enc}{Plain} \\
    \rc{enc}{Cipher}{in}{Msg}
\end{align}

\subsubsection*{Proof}

To show that in the given network all required guarantees for symmetric
encryption are established, we need to proof that encryption integrity
\eqref{eq:enc1}, key integrity \eqref{eq:enc2}, key confidentiality
\eqref{eq:enc3} and counter integrity \eqref{eq:enc4} are true.

\begin{proof}{Encryption integrity}
From $\intg{\invar{\name(in, Msg)}} \equiv
False$, $\intg{\outvar{\name(enc, Cipher)}} \Leftrightarrow
\intg{\invar{\name(in, Msg)}}$ (\ref{eq:encCipherinMsgIntg},\ \ref{eq:in})  have
$\intg{\outvar{\name(enc, Cipher)}} \equiv False$. Using material implication
this proofs \eqref{eq:enc1}.
\end{proof}

\begin{proof}{Key integrity}
From $\intg{\outvar{\name(ks, Key)}} \equiv True$, $\intg{\outvar{\name(ks,
Key)}} \Leftrightarrow \intg{\invar{\name(enc, Key)}}$ (\ref{eq:ks2},
\ref{eq:ksKeyencKeyIntg}) follows $\intg{\invar{\name(enc, Key)}} \equiv True$
\eqref{eq:enc2}. $\square$
\end{proof}

\begin{proof}{Key confidentiality}
From $\conf{\outvar{\name(ks, Key)}} \equiv True$, $\conf{\outvar{\name(ks,
Key)}} \Leftrightarrow \conf{\invar{\name(enc, Key)}}$ (\ref{eq:ks1},
\ref{eq:ksKeyencKeyConf}) follows \eqref{eq:enc3}. $\square$
\end{proof}

\begin{proof}{Counter integrity}
From $\intg{\outvar{\name(iv, Const)}} \Leftrightarrow \intg{\invar{\name(enc, Ctr)}}$ (\ref{eq:iv},
\ref{eq:ivConstencCtrIntg}) follows $\eqref{eq:enc3} \equiv True$.
\end{proof}


==> parts/workflow.tex <==
\subsection{\label{subsec:workflow}Workflow}

\begin{figure}[h]
    \centering
    \tiny\sf
    \makebox[\linewidth][c]{
      \resizebox{1.0\linewidth}{!}{%
        \input{images/workflow.teximg}
      }
    }
    \caption{High-level workflow for creating partitioned cryptographic protocols.
             Dashed parts mark future work items, see \Cref{subsec:future} for
             details.}
    \label{fig:workflow}
\end{figure}

The workflow to obtain a partitioned cryptographic protocol using our
toolset is outlined in\Cref{fig:workflow}. The process starts with the
\emph{Input model}, a machine-readable description of the protocol defining
model primitives, the data flow between primitives and the environment the
protocol interacts with. On the parsed model, an analysis and partitioning step
(cf\Cref{fig:toolset}) verifies whether the security assumptions
defined by the environment and implied by the model are consistent. If this
leads to a contradiction, the user is presented with an annotated model
describing the conflict that was determined. This information can be used to
refine the input unit it is sound. Additionally, the model can be executed
using implementations available with the toolset and user-provided
implementations for model primitives. This allows for further refinement of the
input model to validate its functionality e.g. by running it against
independent reference implementations.

The output model is a version of the input model with primitives grouped into
partitions. Primitives within the same partition do not require any isolation
and can be implemented in the same protection domain (e.g. as functions in the
same process). All primitives and channels in the model are annotated with the
guarantees the system has to provide to them. An implementer can use that to
derive the communication policy within the system and to decide whether a
functionality must be realized in special trusted process or it can be done in
a container running an off-the-shelf software stack.

